BPP-Search: Enhancing Tree of Thought Reasoning for Mathematical Modeling Problem Solving

LLMs exhibit advanced reasoning capabilities, offering the potential to transform natural language questions into mathematical models. However, existing open-source datasets in operations research domain lack detailed annotations of the modeling process, such as variable definitions, focusing solely on objective values, which hinders reinforcement learning applications. To address this, we release the StructuredOR dataset, annotated with comprehensive labels that capture the complete mathematical modeling process. We further propose BPP-Search, an algorithm that integrates reinforcement learning into a tree-of-thought structure using Beam search, a Process reward model, and a pairwise Preference algorithm. This approach enables efficient exploration of tree structures, avoiding exhaustive search while improving accuracy. Extensive experiments on StructuredOR, NL4OPT, and MAMO-ComplexLP datasets show that BPP-Search significantly outperforms state-of-the-art methods. In tree-based reasoning, BPP-Search excels in accuracy and efficiency, enabling faster retrieval of correct solutions. The StructuredOR dataset is available on Huggingface https://huggingface.co/datasets/LLM4OR/StructuredOR and GitHub https://github.com/LLM4OR/StructuredOR.

==> ignore.tex <==
There is an example for the desired data structure.

```
{
    "set": [
      {
        "name": "Targets",
        "description": "Set of radar installations to be destroyed",
        "data": [
          1,
          2,
          3,
          4
        ]
      },
      {
        "name": "Weapons",
        "description": "Set of alternative weapons usable for the mission",
        "data": [
          1,
          2
        ]
      }
    ],
    "parameter": [
      {
        "name": "Firepower",
        "description": "Firepower of weapon `w`",
        "domain": "{w <in> Weapons}",
        "data": [
          7,
          2
        ]
      },
      {
        "name": "Cost",
        "description": "Cost of deploying weapon `w`",
        "domain": "{w <in> Weapons}",
        "data": [
          1008.5,
          1000.5
        ]
      },
      {
        "name": "ReqFirepower",
        "description": "Required firepower to destroy target `t`",
        "domain": "{t <in> Targets}",
        "data": [
          17,
          5,
          9,
          8
        ]
      },
      {
        "name": "AvailWeapons",
        "description": "Number of available weapons of type `w`",
        "domain": "{w <in> Weapons}",
        "data": [
          8,
          11
        ]
      }
    ],
    "variable": [
      {
        "name": "Assignment",
        "description": "Assignment of weapon `w` to target `t`",
        "domain": "{w <in> Weapons, t <in> Targets}",
        "type": "integer"
      }
    ],
    "objective": [
      {
        "name": "TotalCost",
        "description": "Total cost of destroying all targets",
        "sense": "min",
        "function": "<sum>_{w <in> Weapons, t <in> Targets} Cost_{w} * Assignment_{w,t}"
      }
    ],
    "constraint": [
      {
        "name": "FirepowerRequirement",
        "description": "Firepower requirement for each target",
        "domain": "{t <in> Targets}",
        "function": "<sum>_{w <in> Weapons} Firepower_{w} * Assignment_{w,t} >= ReqFirepower_{t}"
      },
      {
        "name": "WeaponUsage",
        "description": "Weapon usage must not exceed the available number",
        "domain": "{w <in> Weapons}",
        "function": "<sum>_{t <in> Targets} Assignment_{w,t} <= AvailWeapons_{w}"
      }
    ]
  }
```

## JSON Field Description

| Name       | Type | Required | Description                                         |
|------------|------|----------|-----------------------------------------------------|
| set        | list | No       | Collection definitions needed for abstract modeling |
| parameter  | list | No       | Constants needed for abstract modeling              |
| variable   | list | Yes      | Variables required for modeling                     |
| objective  | list | Yes      | Objective function definition required for modeling |
| constraint | list | No       | Constraints needed for modeling                     |

## Set

| Name        | Type | Description                                                                                                                                                              |
|-------------|------|--------------------------------------------------------------------------------------------------------------------------------------------------------------------------|
| name        | str  | Collection name, must meet programming naming conventions, no spaces allowed                                                                                             |
| description | str  | Description of the collection                                                                                                                                            |
| data        | list | Use a list starting from 1 and ending at the size of the set to represent the number of elements in the set.                                                             |

## Parameter

| Name        | Type | Description                                                                                                                                                                                                                 |
|-------------|------|-----------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------|
| name        | str  | Parameter name, must meet programming naming conventions, no spaces allowed                                                                                                                                                 |
| description | str  |  Parameter description                                                                                                                                                                                                       |
| domain      | str  |  The index dimension of the parameter, e.g., "{a \<in\> Aircraft}". If this parameter is a constant, the domain is an empty string. If this parameter is multi-dimensional, please list the corresponding index.             |
| data        | list |  Use a list or a number depending on whether the domain is an empty string. If the domain is an empty string, the data is a number. Otherwise, it is a list that can be either one-dimensional or multi-dimensional, representing the values of each parameter across different sets. There is a one-to-one correspondence between the dimensions of data and the domain. 如果domain是空字符串，data一定是number, 如果不是，data一定是list  |

## Variable

| Name        | Type | Description                                                                         |
|-------------|------|-------------------------------------------------------------------------------------|
| name        | str  |  Variable name, must meet programming naming conventions, no spaces allowed          |
| description | str  |  Variable description                                                                |
| domain      | str  | Index dimension of the variable, e.g., "{a \<in\> Aircraft}"                        |
| type        | str  |  Variable type: CONTINUOUS, INTEGER, BINARY. Default is CONTINUOUS. Case insensitive |

## Objective

| Name        | Type | Description                                                                          |
|-------------|------|--------------------------------------------------------------------------------------|
| name        | str  | Objective function name, must meet programming naming conventions, no spaces allowed |
| description | str  |  Objective function description                                                       |
| sense       | str  |  Optimization direction of the objective function: min, max, minimize, maximize       |
| function    | str  | Formula of the objective function, details below                                     |

## Constraint

| Name        | Type | Description                                                                                                                                                          |
|-------------|------|----------------------------------------------------------------------------------------------------------------------------------------------------------------------|
| name        | str  |  Constraint name, must meet programming naming conventions, no spaces allowed                                                                                         |
| description | str  |  Constraint description                                                                                                                                               |
| domain      | str  | Index dimension of the constraint. Without filter: "{a \<in\> Aircraft}".|
| function    | str  |  Formula of the constraint, details below                                                                                                                             |

## Formula Details

| Type                    | Expression              | Description                             |
|-------------------------|-------------------------|-----------------------------------------|
| Formula with sum symbol | `<sum>_{i <in> I} x_{i}` | `{i <in> I}` is the summation dimension |

## Unsupported Formulas

| Type                                   | Expression                                    | Description                             |
|----------------------------------------|-----------------------------------------------|-----------------------------------------|
| Sum dimension with subscript parameter | `<sum>_{i <in> Successors_{k}}`               | Does not support `Successors_{k}` forms |
| Nested parentheses in index dimension  | `{i <in> P {k <in> A l <in> A} <in> NOE_{i}}` |                                         |
| Subscript restriction                  | `X_{i,j}` where `i, j` cannot be a number         | Numeric subscripts like `X_{i,1}`, `X_{1,j}` are not supported |





## Supported Special Formulas

| Type                            | Expression                                  | Description                                                             |
|---------------------------------|---------------------------------------------|-------------------------------------------------------------------------|
| Continuous expression           | `a<b<c`                                     |                                                                         |
| Expression separated by commas  | `x + y < 0, y + z < 1`                      | Must be separated by English commas; will be split into two constraints |
| Two consecutive sums            | `<sum>_{i <in> I} <sum>_{j <in> J} x_{ij}`  | Will be merged into: `<sum>_{i <in> I j <in> J} x_{ij}`                 |
| Missing * multiplication symbol | `<sum>_{i <in> I}(a_{i}x_{i} + b_{i}y_{i})` | Multiplication symbol will be automatically filled                      |


def build_prm_training_data_template(question, label):
    convention = get_the_convention()

    template = f"""As an expert in mathematical modeling, you are provided with the conventions for generating instances from concrete problems. The conventions are as follows:

{convention}

Please review the following question:
{question}

And evaluate the following mathematical model (or part of it):
{label}
"""
    return template


def build_dpo_training_data_template(question, model1, model2):
    convention = get_the_convention()

    template = f"""As an expert in mathematical modeling, you are provided with conventions for generating instances from concrete problems. The conventions are as follows:

{convention}

Please review the following question:
Question: {question}

Evaluate the following two mathematical models:

Model 1 Answer:
{model1}

Model 2 Answer:
{model2}

Instructions:
If Model 1 is correct and Model 2 is incorrect, please consider this example as positive.
If Model 2 is correct and Model 1 is incorrect, please consider this example as negative.
"""
    return template

==> imgs/convention.tex <==
\begin{longtable}[]{@{}
  >{\raggedright\arraybackslash}p{(\columnwidth - 6\tabcolsep) * \real{0.1370}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 6\tabcolsep) * \real{0.0548}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 6\tabcolsep) * \real{0.1096}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 6\tabcolsep) * \real{0.6986}}@{}}
\toprule\noalign{}
\begin{minipage}[b]{\linewidth}\raggedright
Name
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Type
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Required
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Description
\end{minipage} \\
\midrule\noalign{}
\endhead
\bottomrule\noalign{}
\endlastfoot
set & list & No & Collection definitions needed for abstract modeling \\
parameter & list & No & Constants needed for abstract modeling \\
variable & list & Yes & Variables required for modeling \\
objective & list & Yes & Objective function definition required for
modeling \\
constraint & list & No & Constraints needed for modeling \\
\end{longtable}

\paragraph{Set}\label{set}

\begin{longtable}[]{@{}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.1467}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.0533}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.8000}}@{}}
\toprule\noalign{}
\begin{minipage}[b]{\linewidth}\raggedright
Name
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Type
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Description
\end{minipage} \\
\midrule\noalign{}
\endhead
\bottomrule\noalign{}
\endlastfoot
name & str & Collection name, must meet programming naming conventions,
no spaces allowed \\
description & str & Description of the collection \\
data & list & Use a list starting from 1 and ending at the size of the
set to represent the number of elements in the set. \\
\end{longtable}

\paragraph{Parameter}\label{parameter}

\begin{longtable}[]{@{}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.1467}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.0533}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.8000}}@{}}
\toprule\noalign{}
\begin{minipage}[b]{\linewidth}\raggedright
Name
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Type
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Description
\end{minipage} \\
\midrule\noalign{}
\endhead
\bottomrule\noalign{}
\endlastfoot
name & str & Parameter name, must meet programming naming conventions,
no spaces allowed \\
description & str & Parameter description \\
domain & str & The index dimension of the parameter, e.g., ``\{a
\textless in\textgreater{} Aircraft\}''. If this parameter is a
constant, the domain is an empty string. If this parameter is
multi-dimensional, please list the corresponding index. \\
data & list & Use a list or a number depending on whether the domain is
an empty string. If the domain is an empty string, the data is a number.
Otherwise, it is a list that can be either one-dimensional or
multi-dimensional, representing the values of each parameter across
different sets. There is a one-to-one correspondence between the
dimensions of data and the domain. \\
\end{longtable}

\paragraph{Variable}\label{variable}

\begin{longtable}[]{@{}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.1467}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.0533}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.8000}}@{}}
\toprule\noalign{}
\begin{minipage}[b]{\linewidth}\raggedright
Name
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Type
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Description
\end{minipage} \\
\midrule\noalign{}
\endhead
\bottomrule\noalign{}
\endlastfoot
name & str & Variable name, must meet programming naming conventions, no
spaces allowed \\
description & str & Variable description \\
domain & str & Index dimension of the variable, e.g., ``\{a
\textless in\textgreater{} Aircraft\}'' \\
type & str & Variable type: CONTINUOUS, INTEGER, BINARY. Default is
CONTINUOUS. Case insensitive \\
\end{longtable}

\paragraph{Objective}\label{objective}

\begin{longtable}[]{@{}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.1467}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.0533}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.8000}}@{}}
\toprule\noalign{}
\begin{minipage}[b]{\linewidth}\raggedright
Name
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Type
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Description
\end{minipage} \\
\midrule\noalign{}
\endhead
\bottomrule\noalign{}
\endlastfoot
name & str & Objective function name, must meet programming naming
conventions, no spaces allowed \\
description & str & Objective function description \\
sense & str & Optimization direction of the objective function: min,
max, minimize, maximize \\
function & str & Formula of the objective function, details below \\
\end{longtable}

\paragraph{Constraint}\label{constraint}

\begin{longtable}[]{@{}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.1467}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.0533}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.8000}}@{}}
\toprule\noalign{}
\begin{minipage}[b]{\linewidth}\raggedright
Name
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Type
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Description
\end{minipage} \\
\midrule\noalign{}
\endhead
\bottomrule\noalign{}
\endlastfoot
name & str & Constraint name, must meet programming naming conventions,
no spaces allowed \\
description & str & Constraint description \\
domain & str & Index dimension of the constraint. Without filter: ``\{a
\textless in\textgreater{} Aircraft\}''. \\
function & str & Formula of the constraint, details below \\
\end{longtable}

\paragraph{Formula Details}\label{formula-details}

\begin{longtable}[]{@{}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.2674}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.2791}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.4535}}@{}}
\toprule\noalign{}
\begin{minipage}[b]{\linewidth}\raggedright
Type
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Expression
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Description
\end{minipage} \\
\midrule\noalign{}
\endhead
\bottomrule\noalign{}
\endlastfoot
Formula with sum symbol &
\texttt{\textless{}sum\textgreater{}\_\{i\ \textless{}in\textgreater{}\ I\}\ x\_\{i\}}
& \texttt{\{i\ \textless{}in\textgreater{}\ I\}} is the summation
dimension \\
\end{longtable}

\paragraph{Unsupported Formulas}\label{unsupported-formulas}

\begin{longtable}[]{@{}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.2657}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.3147}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.4196}}@{}}
\toprule\noalign{}
\begin{minipage}[b]{\linewidth}\raggedright
Type
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Expression
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Description
\end{minipage} \\
\midrule\noalign{}
\endhead
\bottomrule\noalign{}
\endlastfoot
Sum dimension with subscript parameter &
\texttt{\textless{}sum\textgreater{}\_\{i\ \textless{}in\textgreater{}\ Successors\_\{k\}\}}
& Does not support \texttt{Successors\_\{k\}} forms \\
Nested parentheses in index dimension &
\texttt{\{i\ \textless{}in\textgreater{}\ P\ \{k\ \textless{}in\textgreater{}\ A\ l\ \textless{}in\textgreater{}\ A\}\ \textless{}in\textgreater{}\ NOE\_\{i\}\}}
& \\
Subscript restriction & \texttt{X\_\{i,j\}} where \texttt{i,\ j} cannot
be a number & Numeric subscripts like \texttt{X\_\{i,1\}},
\texttt{X\_\{1,j\}} are not supported \\
\end{longtable}

\paragraph{Supported Special
Formulas}\label{supported-special-formulas}

\begin{longtable}[]{@{}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.2313}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.3209}}
  >{\raggedright\arraybackslash}p{(\columnwidth - 4\tabcolsep) * \real{0.4478}}@{}}
\toprule\noalign{}
\begin{minipage}[b]{\linewidth}\raggedright
Type
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Expression
\end{minipage} & \begin{minipage}[b]{\linewidth}\raggedright
Description
\end{minipage} \\
\midrule\noalign{}
\endhead
\bottomrule\noalign{}
\endlastfoot
Continuous expression & \texttt{a\textless{}b\textless{}c} & \\
Expression separated by commas &
\texttt{x\ +\ y\ \textless{}\ 0,\ y\ +\ z\ \textless{}\ 1} & Must be
separated by English commas; will be split into two constraints \\
Two consecutive sums &
\texttt{\textless{}sum\textgreater{}\_\{i\ \textless{}in\textgreater{}\ I\}\ \textless{}sum\textgreater{}\_\{j\ \textless{}in\textgreater{}\ J\}\ x\_\{ij\}}
& Will be merged into:
\texttt{\textless{}sum\textgreater{}\_\{i\ \textless{}in\textgreater{}\ I\ j\ \textless{}in\textgreater{}\ J\}\ x\_\{ij\}} \\
Missing * multiplication symbol &
\texttt{\textless{}sum\textgreater{}\_\{i\ \textless{}in\textgreater{}\ I\}(a\_\{i\}x\_\{i\}\ +\ b\_\{i\}y\_\{i\})}
& Multiplication symbol will be automatically filled \\
\end{longtable}


==> tables/complex_lp.tex <==
\begin{table}[]
\footnotesize
\caption{
Accuracy and the number of reasoning steps required under different reasoning methods with a fixed policy model (GPT-4o) on the ComeplexLP\cite{complexLP} test dataset, focusing on the 72 problems confirmed solvable by the current policy model based on prior experiments. Note: "PA" denotes the use of a preference algorithm.
}

\centering
\label{tab:complexLP}
\resizebox{\linewidth}{!}{
% \begin{tabular}{l|c|c|c}
\begin{tabular}{l|l|c}
\hline
Method & Correct Rate & Reasoning Steps\\
\hline
CoT & 0.486 & 1 \\
SC & 0.625 & 4 \\
ToT-Randomly-Chosen & 0.444 & 39 \\
ToT-Rethink & 0.583 & 40 \\ \hline

Greedy & 0.555 & 9 \\
Randomly Greedy & 0.527 & 9 \\
Epsilon Greedy & 0.5 & 9 \\ \hline
Beam Search (Width=2) & 0.652 & 15 \\
Beam Search (Width=3) & 0.666 & 21 \\ \hline
Beam Search (Width=2) + PA & 0.652 & 15 \\
Beam Search (Width=3) + PA & 0.722 & 21 \\
\hline


\end{tabular}}
\end{table}

==> tables/nl4opt.tex <==
\begin{table}[]
\footnotesize
\caption{
Accuracy and the number of reasoning steps required under different reasoning methods with a fixed policy model (GPT-4o) on the NL4OPT\cite{nl4opt} test dataset, focusing on the 143 problems confirmed solvable by the current policy model based on prior experiments. Note: "PA" denotes the use of a preference algorithm.
}

\centering
\label{tab:nl4opt}
\resizebox{\linewidth}{!}{
% \begin{tabular}{l|c|c|c}
\begin{tabular}{l|l|c}
\hline
Method & Correct Rate & Reasoning Steps\\
\hline
CoT & 0.566 & 1 \\
SC & 0.713 & 4 \\
ToT-Randomly-Chosen & 0.629 & 39 \\
ToT-Rethink & 0.622 & 40 \\ \hline

Greedy & 0.699 & 9 \\
Randomly Greedy & 0.692 & 9 \\
Epsilon Greedy & 0.713 & 9 \\ \hline
Beam Search (Width=2) & 0.783 & 15 \\
Beam Search (Width=3) & 0.755 & 21 \\ \hline
Beam Search (Width=2) + PA & 0.804 & 15 \\
Beam Search (Width=3) + PA & 0.797 & 21 \\
\hline


\end{tabular}}
\end{table}

==> tables/structuredOR.tex <==
\begin{table}[]
\footnotesize
\caption{
Accuracy and the number of reasoning steps required under different reasoning methods with a fixed policy model (GPT-4o) on the StructuredOR test dataset, focusing on the 30 problems confirmed solvable by the current policy model based on prior experiments. Note: "PA" denotes the use of a preference algorithm.
}

\centering
\label{tab:structureOR}
\resizebox{\linewidth}{!}{
% \begin{tabular}{l|c|c|c}
\begin{tabular}{l|l|c}
\hline
Method & Correct Rate & Reasoning Steps\\
\hline
CoT & 0.633 & 1 \\
SC & 0.7 & 4 \\
ToT-Randomly-Chosen & 0.7 & 39 \\
ToT-Rethink & 0.766 & 40 \\ \hline

Greedy & 0.733 & 9 \\
Randomly Greedy & 0.833 & 9 \\
Epsilon Greedy & 0.733 & 9 \\ \hline
Beam Search (Width=2) & 0.8 & 15 \\
Beam Search (Width=3) & 0.766 & 21 \\ \hline
Beam Search (Width=2) + PA & 0.933 & 15 \\
Beam Search (Width=3) + PA & 0.866 & 21 \\
\hline


\end{tabular}}
\end{table}
